Fast Dual Simulation Processing of Graph Database Queries (Supplement)

Graph database query languages feature expressive, yet computationally expensive pattern matching capabilities. Answering optional query clauses in SPARQL for instance renders the query evaluation problem immediately Pspace-complete. Therefore, light-weight graph pattern matching relations, such as simulation, have recently been investigated as promising alternatives to more expensive query mechanisms like, e.g., computing subgraph isomorphism. Still, graph pattern matching alone lacks expressive query capabilities: all patterns are combined by usual join constructs, where more sophisticated capabilities would be inevitable for making solutions useful to emerging applications. In this paper we bridge this gap by introducing a new dual simulation process operating on SPARQL queries. In addition to supporting the full syntactic structure of SPARQL queries, it features polynomial-time pattern matching to compute an overapproximation of query results from the database. Moreover, to achieve runtimes competing with state-of-the-art database systems, we develop a novel algorithmic solution to dual simulation graph pattern matching, based on a system of inequalities that allows for several optimization heuristics. Finally, we achieve soundness of our process for SPARQL queries including UNION, AND and OPTIONAL operators not restricted to well-designed patterns. Our experiments on synthetic and real-world graph data promise a clear gain for graph database systems when incorporating the new dual simulation techniques. In this supplement paper we present in detail all proofs, discussions of experimental results, and complexity analysis for the original paper "Fast Dual Simulation Processing of Graph Database Queries" included in the Proceedings of the 35th IEEE International Conference on Data Engineering (ICDE 2019), Macau, China.

==> tex/abstract.tex <==
Graph database query languages feature expressive, yet computationally expensive pattern matching capabilities.
Answering optional query clauses in \sparql for instance renders the query evaluation problem immediately \pspace-complete.
Therefore, light-weight graph pattern matching relations, such as simulation, have recently been investigated as promising alternatives to more expensive query mechanisms like, \eg computing subgraph isomorphism.
Still, graph pattern matching alone lacks expressive query capabilities: all patterns are combined by usual join constructs, where more sophisticated capabilities would be inevitable for making solutions useful to emerging applications.
In this paper we bridge this gap by introducing a new {\em dual simulation process} operating on \sparql queries.
In addition to supporting the full syntactic structure of \sparql queries, it features polynomial-time pattern matching to compute an overapproximation of query results from the database.
Moreover, to achieve runtimes competing with state-of-the-art database systems, we develop a novel algorithmic solution to dual simulation graph pattern matching, based on a system of inequalities that allows for several optimization heuristics.
Finally, we achieve soundness of our process for \sparql queries including \sunion, \sand and \soptional operators not restricted to well-designed patterns.
Our experiments on synthetic and real-world graph data promise a clear gain for graph database systems when incorporating the new dual simulation techniques.


==> tex/proofs.tex <==
\subsection{Proof of Lemma~\ref{lemma:bgp-semantics}}
%
%\begin{proof}
$\mu\upharpoonright\vars(\mathcal G)$ restricts match $\mu$ to the variables occurring in $\mathcal G$, \ie $(\mu\upharpoonright\vars(\mathcal G))(v)$ is $\mu(v)$ if $v\in\vars(\mathcal G)$ and undefined otherwise.
A function $f : \vars(G)\to O_\db$ is a graph homomorphism from $Q(\mathcal G)$ to \db iff for each edge $(v_1,a,v_2)$ in $Q(\mathcal G)$ there is an edge $(f(v_1),a,f(v_2))$ in \db.
$\mu\in\lbr\mathcal G\rbr_\db$ iff $\dom(\mu)\subseteq\vars(\mathcal G)$ and $\forall t\in\mathcal G : \mu(t)\in\db$.
For $\nu = \mu\upharpoonright\vars(\mathcal G)$, it follows that for all edges $(v_1,a,v_2)$ of $Q(\mathcal G)$ (\ie $\mathcal G$), $(\nu(v_1),a,\nu(v_2))$ is an edge of \db.
The converse direction follows the backwards line of arguments.
%\end{proof}

\subsection{Proof of Lemma~\ref{lemma:bgp-completeness}}
%
%\begin{proof}
Let $Q=(\vars(\mathcal G),\Sigma,\mathcal G,\{ g \})$ be the query graph of $\mathcal G$ and $S$ the largest dual simulation between $Q$ and \db.
By Lemma~\ref{lemma:bgp-semantics}, every match $\mu\in\lbr\mathcal G\rbr_\db$ is a homomorphism.
Furthermore, if every homomorphism is a dual simulation and since the largest dual simulation is unique, for every match $\mu$, it holds that $\mu\subseteq S$.
Thus, $\db(Q,S)$ is $\mathcal G$-complete.

It remains to be shown that every homomorphism $f$ indeed is a dual simulation between the respective graphs.
Let $G_1$ and $G_2$ be two graphs and $f$ a homomorphism from $G_1$ to $G_2$, \ie $f : V_1 \to V_2$ such that for every edge $v_1 \transrel{a}_1 v_2$, $f(v_1) \transrel{a}_2 f(v_2)$.
For $(v_1,f(v_1))\in f$, the forwards edge condition (first bullet in Def.~\ref{def:dual-simulation}) directly follows.
For the second condition, we rely on the fact that $f$ is a function, thus relates every node from $V_1$ with some node from $V_2$.
Suppose now we have $v_2 \transrel{a}_\db v_1$.
Since $f$ is a function and a graph homomoporphism, it follows that $f(v_2)\transrel{a}_2 f(v_1)$.
Thus, there is a $w_2$ such that $w_2 \transrel{a}_2 f(v_1)$, namely $w_2 = f(v_2)$.
%\end{proof}
%

\subsection{Proof of Proposition~\ref{prop:query-simulation}}
%
%\begin{proof}
For claim (1), we assume $S_1$ and $S_2$ to be query graph simulations with respective pre-simulations $P_1$ and $P_2$.
The pre-simulation proving $S_1 \cup S_2$ to be a query graph simulation shall be $P_1\cup P_2$.
Whenever we have only disjoint groups handled by $P_1$ and $P_2$, $P_1\cup P_2$ is a pre-simulation, since $P_1$ and $P_2$ are.
For groups $g$ jointly incorporated in $P_1$ and $P_2$, for $(v_1, g, w_1)\in P_1 \cup P_2$, $v_1 \transrel{a}_g v_2$ must be complemented by a $w_2$ such that $w_1 \transrel{a}_g w_2$ and $(v_2,g,w_2)\in P_1 \cup P_2$.
But this step stems must be justified by $P_1$ or $P_2$ and since $P_i \subseteq P_1 \cup P_2$, $(v_2,g,w_2)\in P_1\cup P_2$.
For backwards edges, we follow a similar line of arguments.
%Since dual simulation is closed under union~\cite{Ma2014}, $P_1\cup P_2$ is a pre-simulation.

For query graph $Q=(V,\Sigma,\transrel{},\Gamma)$ and graph database \db, let $P_g$ be the largest pre-simulations between group $g\in\Gamma$ and \db.
We derive from $P_g$ a dual simulation $S_g$ by removing the group component from $P_g$.
As Ma \etal~\cite{Ma2014} have shown, all $S_g$ are unique and, hence, also all $P_g$ are unique.
The largest query graph simulation $S=\bigcup_{g\in \Gamma} S_g$ is thus unique.
% $S$ being not unique contradicts the assumption that all $S_g$ are unique.
%\end{proof}
%

\subsection{Proof of Lemma~\ref{lemma:match-dualsim}}
%
%\begin{proof}
We prove the claim by induction over the structure of \Q.
Let therefore $\mu\in\lbr\Q\rbr_\db$.
\begin{description}
\item[Base:] For \Q being a BGP, $\mu$ is a query graph simulation iff it is a dual simulation, since there is only a single group in \Q.
In Lemma~\ref{lemma:bgp-completeness}, we have shown that $\mu$ in this case is a dual simulation. 
\item[Step:] Assume for \Q[1] and \Q[2], every $\mu\in\lbr\Q[i]\rbr_\db$ ($i=1,2$) is a query graph simulation.
It remains to be shown that matches $\mu$ to $\Q=\Q[1]\sop\Q[2]$ ($\sop\in\{\sand,\sunion,\soptional\}$) also are query graph simulations.
In case of $\sop=\sunion$, the claim follows by the induction hypothesis, since $\mu\in\lbr\Q\rbr_\db$ iff $\mu\in\lbr\Q[1]\rbr_\db\cup\lbr\Q[2]\rbr_\db$.
In case of $\sop=\sand$, we have that $\mu\in\lbr\Q\rbr_\db$ iff there are compatible $\mu_i\in\lbr\Q[i]\rbr_\db$ ($i=1,2$) and $\mu=\mu_1\cup\mu_2$.
By Proposition~\ref{prop:query-simulation}(1), query graph simulation is closed under union, thus making $\mu$ a query graph simulation.
The last case, $\sop=\soptional$, follows directly from the induction hypothesis (in case $\mu=\mu_1$ with $\mu_1 \in\lbr\Q[1]\rbr_\db$ with no compatible match in \Q[2]) or from the argumentation on $\sop=\sand$ (in case there are compatible matches).
\end{description}
%\end{proof}

\subsection{Proof of Proposition~\ref{prop:join-completeness}}
%
%\begin{proof}
We need to show that for each variable $x\in\vars(\Q)$ and each match $\mu\in\lbr\Q\rbr_\db$ with $\mu(x)$ defined, it holds that $(x,\mu(x))\in S$.
We distinguish two cases.
First, $x$ is not shared between \Q[1] and \Q[2].
W.\,l.\,o.\,g.\xspace, $x\in\vars(\Q[1])$ and there is a match $\mu_1\in\lbr\Q[1]\rbr_\db$ with $\mu_1(x)=\mu(x)$.
Since $\db(Q(\Q[1]),S_1)$ is \Q[1]-complete \wrt \db, $(x,\mu_1(x))\in S_1$.
As $x\notin\vars(\Q[1])\cap\vars(\Q[2])$, it follows that $(x,\mu(x))\in S$.
As the second case, consider $x$ to be shared between \Q[1] and \Q[2].
Thus, there exist compatible matches $\mu_i \in\lbr\Q[i]\rbr_\db$ ($i=1,2$) such that $\mu_1(x)=\mu_2(x)=\mu(x)$.
Since $\db(Q(\Q[i]),S_i)$ is \Q[i]-complete \wrt \db, $(x,\mu_i(x))\in S_i$ ($i=1,2$).
Hence, also $S_1$ and $S_2$ agree on $(x,\mu(x))$ and therefore $(x,\mu(x))\in S$.
%\end{proof}

\subsection{Proof of Proposition~\ref{prop:optional-completeness}}
%
We need to show that for each variable $x\in\vars(\Q)$ and each match $\mu\in\lbr\Q\rbr_\db$ with $\mu(x)$ defined, it holds that $(x,\mu(x))\in S$.
We distinguish again two cases.
First, $x$ is no shared variable between \Q[1] and \Q[2] and second, $x$ is a shared variable.
For the first case, w.\,l.\,o.\,g.\xspace, $x\in\vars(\Q[1])$ and there is a match $\mu_1\in\lbr\Q[1]\rbr_\db$ with $\mu_1(x)=\mu(x)$.
Since $\db(Q(\Q[1]),S_1)$ is \Q[1]-complete \wrt \db, $(x,\mu_1(x))\in S_1$.
As $x\notin\vars(\Q[1])\cap\vars(\Q[2])$, it follows that $(x,\mu(x))\in S$.
For the second case, $x$ is shared between \Q[1] and \Q[2].
Thus, there exist compatible matches $\mu_i \in\lbr\Q[i]\rbr_\db$ ($i=1,2$) such that $\mu_1(x)=\mu_2(x)=\mu(x)$.
Since $\db(Q(\Q[i]),S_i)$ is \Q[i]-complete \wrt \db, $(x,\mu_i(x))\in S_i$ ($i=1,2$).
Hence, also $S_1$ and $S_2$ agree on $(x,\mu(x))$ and therefore $(x,\mu(x))\in S$.

\subsection{Proof of Proposition~\ref{prop:connectedness}}
%
We prove claim (1) by induction over the shape of \Q.
For the base case, it holds that any match $\mu$ yields a connected graph $\mu(\Q)$, since $Q(\Q)$ is a connected graph and $\mu$ is a homomorphism (\cf Lemma~\ref{lemma:bgp-semantics}).
For disjunction and conjunction, connectedness of $\mu(\Q)$ directly follows from the induction hypothesis.
It remains to be shown that also for optional pattern, $\Q=\Q[1]\soptional\Q[2]$ connectedness of the matches holds as well.
Towards a contradiction, assume there is a match $\mu$ such that $\mu(\Q)$ is disconnected.
Since by induction hypothesis, there are no matches $\mu_i$ to $\Q[i]$ such that $\mu_i(\Q[i])$ is disconnected, there must be compatible $\mu_i$ ($i=1,2$) and one shared variable $v$ defined for $\mu_i$ but not for $\mu_j$ ($i\neq j$).
In any case, $\Q[i]$ has an optional pattern as a sub-query such that the assignment of objects to node $v$ is optional within $\Q[i]$.
Since $v$ is a variable of \Q[j], we obtain a contradiction as \Q cannot be well-designed although it is assumed to be.
Hence, $\mu(\Q)$ being disconnected contradicts the assumption of \Q being a connected query.

In order to prove claim (2), we recall that the diameter of a graph is the longest distance between any two nodes.
Hence, for two nodes $v, v'$ in $\mu(\Q)$, the distance between $v$ and $v'$ is bounded by the diameter of $\mu(\Q)$.
As \Q is a connected query, $\dia(\mu(\Q))=\dia(Q(\Q))=d\in\mathbb{N}$.
Hence, we may follow that $\mu(\Q)$ is a subgraph of each ball $\widehat{\db}[v,d]$ ($v\in V$).


==> tex/queries.tex <==
\subsection{LUBM Queries}
\noindent\textbf{PREFIX} ub: <http://www.lehigh.edu/~zhp2/2004/0401/univ-bench.\\owl\#> 

\noindent\textbf{PREFIX} rdf: <http://www.w3.org/1999/02/22-rdf-syntax-ns\#>\\
\\
%
\noindent\begin{tabular}{l p{7.5cm}}
Q1 &
\textbf{SELECT} * \textbf{WHERE} \{
\{ ?st ub:teachingAssistantOf ?course .
\textbf{OPTIONAL} \{ ?st ub:takesCourse ?course2 . ?pub1 ub:publicationAuthor ?st . \} \} 
\{ ?prof ub:teacherOf ?course . ?st ub:advisor ?prof . 
\textbf{OPTIONAL} \{ ?prof ub:researchInterest ?resint . ?pub2 ub:publicationAuthor ?prof . \} \} \}
\end{tabular}
%
\noindent\begin{tabular}{l p{7.5cm}}
Q2 &
\textbf{SELECT} * \textbf{WHERE} \{
\{ ?pub rdf:type ub:Publication . ?pub ub:publicationAuthor ?st . ?pub ub:publicationAuthor ?prof . 
\textbf{OPTIONAL} \{ ?st ub:emailAddress ?ste .  ?st ub:telephone ?sttel . \} \}
\{ ?st ub:undergraduateDegreeFrom ?univ .  ?dept ub:subOrganizationOf ?univ . 
\textbf{OPTIONAL} \{ ?head ub:headOf ?dept . ?others ub:worksFor ?dept . \} \}
\{ ?st ub:memberOf ?dept . ?prof ub:worksFor ?dept . 
\textbf{OPTIONAL} \{ ?prof ub:doctoralDegreeFrom ?univ1 . ?prof ub:researchInterest ?resint1 . \} \} \}
\end{tabular}
%
\noindent\begin{tabular}{l p{7.5cm}}
Q3 &
\textbf{SELECT} * \textbf{WHERE} \{
\{ ?pub ub:publicationAuthor ?st . ?pub ub:publicationAuthor ?prof . ?st rdf:type ub:GraduateStudent .
\textbf{OPTIONAL} \{ ?st ub:undergraduateDegreeFrom ?univ1 . ?st ub:telephone ?sttel . \} \}
\{ ?st ub:advisor ?prof . 
\textbf{OPTIONAL} \{ ?prof ub:doctoralDegreeFrom ?univ .  ?prof ub:researchInterest ?resint . \} \}
\{ ?st ub:memberOf ?dept . ?prof ub:worksFor ?dept . ?prof rdf:type ub:FullProfessor . 
\textbf{OPTIONAL} \{ ?head ub:headOf ?dept . ?others ub:worksFor ?dept . \} \} \}
\end{tabular}
%
\noindent\begin{tabular}{l p{7.5cm}}
Q4 &
\textbf{SELECT} * \textbf{WHERE} \{
?x ub:worksFor <http://www.Department9.University9999.edu> . ?x rdf:type ub:FullProfessor .
\textbf{OPTIONAL} \{ ?y ub:advisor ?x . ?x ub:teacherOf ?z . ?y ub:takesCourse ?z . \} \}
\end{tabular}
%
\noindent\begin{tabular}{l p{7.5cm}}
Q5 &
\textbf{SELECT} * \textbf{WHERE} \{ 
\{ ?x ub:worksFor <http://www.Department0.University12.edu> . ?x rdf:type ub:FullProfessor . 
\textbf{OPTIONAL} \{ ?y ub:advisor ?x . ?x ub:teacherOf ?z . ?y ub:takesCourse ?z . \} \} \}
\end{tabular}
%
\noindent\begin{tabular}{l p{7.5cm}}
Q6 &
\textbf{SELECT} * \textbf{WHERE} \{ 
?x ub:worksFor <http://www.Department0.University12.edu> . ?x rdf:type ub:FullProfessor . 
\textbf{OPTIONAL} \{ ?x ub:emailAddress ?y1 . ?x ub:telephone ?y2 . ?x ub:name ?y3 . \} \}
\end{tabular}

\subsection{DBpedia Queries}
\noindent\textbf{PREFIX} foaf: <http://xmlns.com/foaf/0.1/> 

\noindent\textbf{PREFIX} geo: <http://www.w3.org/2003/01/geo/wgs84pos\#> 

\noindent\textbf{PREFIX} rdfs: <http://www.w3.org/2000/01/rdf-schema\#> 

\noindent\textbf{PREFIX} dbpowl: <http://dbpedia.org/ontology/> 

\noindent\textbf{PREFIX} dbpprop: <http://dbpedia.org/property/> 

\noindent\textbf{PREFIX} georss: <http://www.georss.org/georss/> 

\noindent\textbf{PREFIX} skos: <http://www.w3.org/2004/02/skos/core\#> 
\\\\
\noindent\begin{tabular}{l p{7.5cm}}
Q7 &
\textbf{SELECT} * \textbf{WHERE} \{ \{ ?v6 rdf:type dbpowl:PopulatedPlace .  ?v6 dbpowl:abstract ?v1 .  ?v6 rdfs:label ?v2 .  ?v6 geo:lat ?v3 .  ?v6 geo:long ?v4 . OPTIONAL \{ ?v6 foaf:depiction ?v8 . \} \} \textbf{OPTIONAL} \{ ?v6 foaf:homepage ?v10 . \} \textbf{OPTIONAL} \{ ?v6 dbpowl:populationTotal ?v12 . \} OPTIONAL \{ ?v6 dbpowl:thumbnail ?v14 . \} \}
\end{tabular}

\noindent\begin{tabular}{l p{7.5cm}}
Q8 &
\textbf{SELECT} * \textbf{WHERE} \{ ?v3 foaf:page ?v0 . ?v3 rdf:type dbpowl:SoccerPlayer .  ?v3 dbpprop:position ?v6 .  ?v3 dbpprop:clubs ?v8 .  ?v8 dbpowl:capacity ?v1 . ?v3 dbpowl:birthPlace ?v5 . \textbf{OPTIONAL} \{ ?v3 dbpowl:number ?v9 . \} \}
\end{tabular}

\noindent\begin{tabular}{l p{7.5cm}}
Q9 &
\textbf{SELECT} * \textbf{WHERE} \{ ?v5 dbpowl:thumbnail ?v4 . ?v5 rdf:type dbpowl:Person . ?v5 rdfs:label ?v . ?v5 foaf:page ?v8 . \textbf{OPTIONAL} \{ ?v5 foaf:homepage ?v10 . \} \}
\end{tabular}

\noindent\begin{tabular}{l p{7.5cm}}
Q10 &
\textbf{SELECT} * \textbf{WHERE} \{ \{ ?v2 rdf:type dbpowl:Settlement . ?v2 rdfs:label ?v . ?v6 rdf:type dbpowl:Airport . ?v6 dbpowl:city ?v2 . ?v6 dbpprop:iata ?v5 . \textbf{OPTIONAL} \{ ?v6 foaf:homepage ?v7 . \} \} \textbf{OPTIONAL} \{ ?v6 dbpprop:nativename ?v8 . \} \}
\end{tabular}

\noindent\begin{tabular}{l p{7.5cm}}
Q11 &
\textbf{SELECT} * \textbf{WHERE} \{ ?v4 skos:subject ?v . ?v4 foaf:name ?v6 . \textbf{OPTIONAL} \{ ?v4 rdfs:comment ?v8 . \} \}
\end{tabular}

\noindent\begin{tabular}{l p{7.5cm}}
Q12 &
\textbf{SELECT} * \textbf{WHERE} \{ ?v0 rdfs:comment ?v1 .  ?v0 foaf:page ?v . \textbf{OPTIONAL} \{ ?v0 skos:subject ?v6 . \} \textbf{OPTIONAL} \{ ?v0 dbpprop:industry ?v5 . \} \textbf{OPTIONAL} \{ ?v0 dbpprop:location ?v2 . \} \textbf{OPTIONAL} \{ ?v0 dbpprop:locationCountry ?v3 . \} \textbf{OPTIONAL} \{ ?v0 dbpprop:locationCity ?v9 . ?a dbpprop:manufacturer ?v0 . \} \textbf{OPTIONAL} \{ ?v0 dbpprop:products ?v11 . ?b dbpprop:model ?v0 . \} \textbf{OPTIONAL} \{ ?v0 georss:point ?v10 . \} \textbf{OPTIONAL} \{ ?v0 rdf:type ?v7 . \} \}
\end{tabular}
\subsection{Additional LUBM Queries}
\noindent\textbf{PREFIX} ub: <http://www.lehigh.edu/~zhp2/2004/0401/univ-bench.\\owl\#> 
\\\\
\noindent\begin{tabular}{l p{7.5cm}}
Q13 &
\textbf{SELECT} *
\textbf{WHERE} \{
    ?pub ub:publicationAuthor ?prof .
    ?prof ub:worksFor ?dep .
    ?dep ub:subOrganizationOf ?uni1 .
    ?st ub:advisor ?prof2. 
    ?st ub:undergraduateDegreeFrom ?uni1 .
    ?prof ub:researchInterest ?reint.
    ?prof3 ub:researchInterest ?reint. 
    ?prof3 ub:worksFor ?dep2 .
    ?dep2 ub:subOrganizationOf ?uni2 .
 \}
\end{tabular}

\noindent\begin{tabular}{l p{7.5cm}}
Q14 &
\textbf{SELECT} *
\textbf{WHERE} \{
    \{?pub ub:publicationAuthor ?prof . \}
    \{?prof ub:worksFor ?dep . \}
    \{?dep ub:subOrganizationOf ?uni1 . \}
    \{?st ub:advisor ?prof2 . \}
    \{?st ub:undergraduateDegreeFrom ?uni1 . \}
    \{?prof ub:researchInterest ?reint . \}
    \{?prof3 ub:researchInterest ?reint . \}
    \{?prof3 ub:worksFor ?dep2 . \}
    \{?dep2 ub:subOrganizationOf ?uni2 . \}
 \}
\end{tabular}

\noindent\begin{tabular}{l p{7.5cm}}
Q15 &
\textbf{SELECT} *
\textbf{WHERE} \{
    \{?pub ub:publicationAuthor ?prof . \}
    \textbf{OPTIONAL} \{?prof ub:worksFor ?dep . \}
    \textbf{OPTIONAL} \{?dep ub:subOrganizationOf ?uni1 . \}
    \textbf{OPTIONAL} \{?st ub:advisor ?prof2 . \}
    \textbf{OPTIONAL} \{?st ub:undergraduateDegreeFrom ?uni1 . \}
    \textbf{OPTIONAL} \{?prof ub:researchInterest ?reint . \}
    \textbf{OPTIONAL} \{?prof3 ub:researchInterest ?reint . \}
    \textbf{OPTIONAL} \{?prof3 ub:worksFor ?dep2 . \}
    \textbf{OPTIONAL} \{?dep2 ub:subOrganizationOf ?uni2 . \} 
 \}
\end{tabular}

\noindent\begin{tabular}{l p{7.5cm}}
Q16 &
\textbf{SELECT} *
\textbf{WHERE} \{
    \{?pub ub:publicationAuthor ?prof . \}
    \textbf{OPTIONAL} \{?prof ub:worksFor ?dep .
    \textbf{OPTIONAL} \{?dep ub:subOrganizationOf ?uni1 .
    \textbf{OPTIONAL} \{?st ub:advisor ?prof2. 
    \textbf{OPTIONAL} \{?st ub:undergraduateDegreeFrom ?uni1 .
    \textbf{OPTIONAL} \{?prof ub:researchInterest ?reint.
    \textbf{OPTIONAL} \{?prof3 ub:researchInterest ?reint. 
    \textbf{OPTIONAL} \{?prof3 ub:worksFor ?dep2 .
    \textbf{OPTIONAL} \{?dep2 ub:subOrganizationOf ?uni2 . \} \} \} \} \} \} \} \}
 \}
\end{tabular}

